Estimating nested expectations without inner conditional sampling and application to value of information analysis

Motivated by various computational applications, we investigate the problem of estimating nested expectations. Building upon recent work by the authors, we propose a novel Monte Carlo estimator for nested expectations, inspired by sparse grid quadrature, that does not require sampling from inner conditional distributions. Theoretical analysis establishes an upper bound on the mean squared error of our estimator under mild assumptions on the problem, demonstrating its efficiency for cases with low-dimensional outer variables. We illustrate the effectiveness of our estimator through its application to problems related to value of information analysis, with moderate dimensionality. Overall, our method presents a promising approach to efficiently estimate nested expectations in practical computational settings.

==> 30-theoretical.tex <==

\section{Theoretical Analysis}\label{sec:theoretical}

In this section, we provide an upper bound on the MSE of our proposed method (Algorithm~\ref{alg:proposed}). We begin by introducing our notation for variance. Throughout this section, given a random vector $Z$, we define the variance of $Z$ as the trace of the covariance matrix of $Z$ and denote it by $\mathbb{V}_{\rho(Z)}Z$. This notation also applies to the case of conditional variance, where we use an appropriate subscript to represent the underlying conditional distribution. Moreover, whenever the underlying probability distribution is clear from the context, we omit the subscript from $\mathbb{E}$ or $\mathbb{V}$ or simply denote the underlying random variables for the subscript instead of the probability distribution. 

As the main theoretical result of this paper, we show the following theorem.
\begin{theorem}\label{thm:main}
    Let $m\in \mathbb{N}$ and $N = 2^m$.
    Assume that $\sup_{Y}\mathbb{V}_{X|Y}g\left(X, Y\right)<\infty$, and there exist positive constants $\alpha_1, \alpha_2, \beta$ and functions $\mathcal{T}_k: \mathbb{R}\to [0,1]$ for all $k=1,\dots, K$, such that
    \begin{enumerate}
        \item $\left| f\left( g \right) - f\left( g + h \right) \right| \leq \alpha_1 \left\| h \right\|_2$,
        \item $\left|f\left( g \right)-f\left( g + h \right)-f\left( g + h' \right)+f\left( g + h + h' \right)\right|\leq \alpha_2 \left\| h \right\|_2 \left\| h' \right\|_2$,
        \item \tg{$\left(\mathbb{E}_{X|Y, X'|Y'}\left\|g\left( X, Y \right) - g\left( X', Y' \right)\right\|^2_2\right)^{1/2} \leq \beta\left\| \mathcal{T}(Y) - \mathcal{T}(Y') \right\|_2$,}
    \end{enumerate}
    for all $g, h, h' \in \mathbb{R}^G$ and $Y, Y' \in \mathbb{R}^K$, in which we write $\mathcal{T}(Y)=(\mathcal{T}_1(Y_1),\dots,\mathcal{T}_K(Y_K)).$
    Then we have
    \begin{align}
        \mathbb{E}(I - \hat{I})^2
    =
        O\left( \frac{(\log N)^2}{N^{1/K}} \right).
    \end{align}
\end{theorem}

Before going into the proof of the theorem, let us make some remarks.
\begin{remark}\label{rem:T_k}
The assumption of the existence of functions $\mathcal{T}_k$ may appear artificial. To argue that this is not the case, let us consider the following change of variables: for $k=1,\dots,K$, let $F_k$ denote the cumulative marginal distribution function of the outer variable $Y_k$ and let $Z_k=F_k(Y_k)$. This transformation ensures that $0 \leq Z_k \leq 1$. Therefore, a natural choice for $\mathcal{T}_k$ is $\mathcal{T}_k=F_k$.

Besides, the condition on $g$ given in the third item of Theorem~\ref{thm:main} implies that
\[ \left\|\mathbb{E}_{X|Y}g\left( X, Y \right) - \mathbb{E}_{X'|Y'}g\left( X', Y' \right)\right\|_2 \leq \beta\left\| \mathcal{T}(Y) - \mathcal{T}(Y') \right\|_2\]
holds for all $Y, Y' \in \mathbb{R}^K$.
\end{remark}

\begin{remark}
If the outer function $f$ satisfies the first condition, it also satisfies
\begin{align*}
    \left|f\left( g \right)-f\left( g + h \right)-f\left( g + h' \right)+f\left( g + h + h' \right)\right| \leq 2\alpha_1\min\left\{ \left\| h \right\|_2,\left\| h' \right\|_2\right\}\leq 2\alpha_1\left( \left\| h \right\|_2 \left\| h' \right\|_2\right)^{1/2}.
\end{align*}
Therefore, it is clear that the second condition imposes a stronger property for $f$.

Theorem~\ref{thm:main} does not necessarily cover the problem setting for estimating EVSI. In fact, for the case where $f=\max_{d\in D}$ for a set $D$ with finite cardinality $G$, it can be checked that the first condition on $f$ is satisfied:
\begin{align*}
    \left| \max_{1\leq j\leq G}g_j-\max_{1\leq j\leq G}(g_j+h_j)\right|\leq \max_{1\leq j\leq G}\left| g_j-(g_j+h_j)\right|\leq \sum_{j=1}^{G}\left| h_j\right|\leq \sqrt{G}\, \|h\|_2,
\end{align*}
where the last inequality follows from Cauchy–Schwarz inequality. However, the second condition on $f$ is not satisfied. Therefore, discussing whether the conditions given in Theorem~\ref{thm:main} can be weakened such that the theorem covers the EVSI setting remains an open problem.
\end{remark}

As a preparation for proving Theorem~\ref{thm:main}, we present the following lemma.
\begin{lemma}\label{lem}
    Let $m \in \mathbb{N}$, and let $\{(X^{(i)}, Y^{(i)})\}_{1 \leq i \leq 2^m}$ be a set of i.i.d.\ random samples from the joint distribution $\rho(X,Y)$. For $d \in \{0, \dots, m\}$ and $\mathbf{u} \in \{0,1\}^d$, let $B^{d}_{\mathbf{u}}$ be constructed as described in Algorithm~\ref{alg:proposed}. Then, assuming the existence of functions $\mathcal{T}_k: \mathbb{R}\to [0,1]$ for all $k=1,\dots, K$  we have for any $d \in \{0, \dots, m\}$
    \begin{align}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \leq
        \frac{2K}{2^{d/K}}.
    \end{align}
\end{lemma}

\begin{proof}
    Let $N=2^m$. For $d \in \{0, \dots, m\}$ and $k\in \{1,\dots, K\}$, define
    \begin{align}
        W_{d, k}
    =
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right).
    \end{align}
    
    If $d = 0$, it is easy to see from the definition $B^0_{\emptyset}:=\{1,\dots,2^m\}$ that
    \begin{align}
        W_{0, k}
    =
        \max_{i \in B^0_{\emptyset}}
        \mathcal{T}_k(Y_k^{(i)})
    -
        \min_{i \in B^0_{\emptyset}}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \max_{ i=1, \dots, 2^m }
        \mathcal{T}_k(Y_k^{(i)})
    -
        \min_{ i=1, \dots, 2^m }
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        1
    \end{align}
    holds for all $k\in\{1,\dots,K\}$.
    
    Otherwise if $1 \leq d \leq m$, it follows from the construction of $B^{d}_{\mathbf{u}}$'s that, for $k = (d-1 \bmod K) +1 \in \{1,\dots,K\}$, we have
    \begin{align}
    & 
        \min_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \min_{i \in B_{\mathbf{u}{:}0}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}0}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \\ &\quad \quad \leq
        \min_{i \in B_{\mathbf{u}{:}1}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}1}^d}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \max_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \end{align}
    for all $\mathbf{u} \in \{0, 1\}^{d-1}$. Therefore, we obtain
    \begin{align}
        W_{d, k} &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        +
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        \right)
    \\ &\leq
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \max_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right) =
        \frac{1}{2}
        W_{d-1, k}.
    \end{align}
    For $k \neq (d-1 \bmod K) +1 $, we have
    \begin{align}
    \quad
        \min_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \min_{i \in B_{\mathbf{u}{:}p}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}p}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \end{align}
    for all $\mathbf{u} \in \{0, 1\}^{d-1}$ and $p \in \{0, 1\}$. Therefore, we obtain
    \begin{align}
     W_{d, k} &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        +
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        \right)
    \\ &\leq
        \frac{2}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \max_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right) =
        W_{d-1, k}.
    \end{align}
    Using these results, it can be concluded that, for any $k\in \{1,\dots,K\}$, we have
    \begin{align}
        W_{d, k} \leq \begin{cases} 1 & \text{if $d < K$,}\\ W_{d-K, k}/2 & \text{otherwise.} \end{cases}
    \end{align}
    so that it holds that
    \begin{align}
            W_{d, k}
        \leq
            \frac{1}{2^{\lfloor d/K \rfloor}}
            W_{d-K\lfloor d/K \rfloor, k}
        \leq
            \frac{1}{2^{\lfloor d/K \rfloor}}
        \leq
            \frac{2}{2^{d/K}},
    \end{align}
    for any $1\leq d\leq m$. Note that this upper bound on $W_{d, k}$ also applies to the case $d=0$.

    Recalling the assumption that $0 \leq \mathcal{T}_k(Y_k) \leq 1$ for any $Y_k$ for all $k=1,\dots, K$, we have for any $d \in \{0, \dots, m\}$
    \begin{align}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2 &\leq
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_1
    \\ &\leq
        \frac{1}{2^d}
        \sum_{k=1}^{K}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left|
            \mathcal{T}_k(Y_k^{(i)})
        -
            \mathcal{T}_k(Y_k^{(j)})
        \right|
    \\ &=
        \frac{1}{2^d}
        \sum_{k=1}^{K}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \sum_{k=1}^{K}
        W_{d, K} \leq
        \frac{2K}{2^{d/K}},
    \end{align}
    which completes the proof of the lemma.
\end{proof}

Let us now prove Theorem~\ref{thm:main}.

\begin{proof}[Proof of Theorem~\ref{thm:main}]
    Together with the notation used in Section~\ref{sec:method}, we further introduce the following notation in this proof:
    \begin{align*}
        \hat{P}_{\mathrm{in}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}f\left(\frac{1}{2^{m-d}}\sum_{i \in B^d_{\mathbf{u}}}\mathbb{E}_{X|Y^{(i)}}g\left(X, Y^{(i)}\right)\right), \\
        \hat{Q}_{\mathrm{in}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}f\left(\frac{1}{2^{m-d}}\sum_{i \in B'^d_{\mathbf{u}}}\mathbb{E}_{X|Y^{(i)}}g\left(X, Y^{(i)}\right)\right), \\
        \hat{P}_{\mathrm{out}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}\mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}f\left(\frac{1}{2^{m-d}}\sum_{i \in B^d_{\mathbf{u}}}g\left(X^{(i)}, Y^{(i)}\right)\right), \\
        \hat{Q}_{\mathrm{out}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}\mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}f\left(\frac{1}{2^{m-d}}\sum_{i \in B'^d_{\mathbf{u}}}g\left(X^{(i)}, Y^{(i)}\right)\right).
    \end{align*}
    Then, by using a trivial inequality $(a+b+c)^2\leq 3(a^2+b^2+c^2)$ for any $a,b,c\in \mathbb{R}$, which follows immediately from Cauchy–Schwarz inequality, we have
    \begin{align}
    &\quad
        \mathbb{E}(I - \hat{I})^2
    \\ &=
        \mathbb{E}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        3
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\quad\quad
    +
        3
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\quad\quad
    +
        3
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2.\label{eq:main_theorem_three_terms}
    \end{align}
In the following, we derive an upper bound on each of the three terms of \eqref{eq:main_theorem_three_terms}. 

\noindent \underline{A bound on the first term of \eqref{eq:main_theorem_three_terms}:}
We start by considering the first term. Applying Cauchy–Schwarz inequality again, we obtain
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &=\mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        -
            \sum_{d=1}^{m}
                \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (m+1)
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    +
        (m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2.
    \end{align}
For the first term on the right-most side above, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
             \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            f\left(
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        \right)^2 
        =
        \frac{1}{2^m}
        \mathbb{V}_{Y}
        f\left(
            \mathbb{E}_{X|Y}
            g(X, Y)
        \right).
    \end{align}
Regarding each summand of the second term, applying Jensen's inequality and using the first condition on $f$ and the exchangeability of the samples $\{Y^{(i)}\}_i$, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
        \frac{1}{2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
            \left(
            f\left(
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
            \right.
        \right.
    \\ & \quad\quad
        -
            \left.
            \left.
            \frac{1}{2}
            \sum_{p \in \{0, 1\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
            \right)
        \right)^2
    \\ & \leq 
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}
    \\ & \quad\quad
        \left(
            f\left(
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ & \leq 
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}
        \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        -
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        \right\|_2^2
    \\ & =
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}\sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}\mathbb{E}_{\sigma|\{Y^{(i)}\}}
    \\ &\quad\quad
        \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        -
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(\sigma(i))}}
                g\left(
                    X, Y^{(\sigma(i))}
                \right)
        \right\|_2^2,
    \end{align}
    where, conditioned on $\{Y^{(i)}\}$, $\sigma$ denotes a random permutation of the indices $1,\dots,2^m$ such that $\sigma(B^{d-1}_{\mathbf{u}})=B^{d-1}_{\mathbf{u}}$. By construction of $B'^{d}_{\mathbf{u}{:}p}$ and because of the restriction $\sigma(B^{d-1}_{\mathbf{u}})=B^{d-1}_{\mathbf{u}}$, the set  $\{Y^{(\sigma(i))}\}_{i \in B'^{d}_{\mathbf{u}{:}p}}$ can be regarded as a set of the samples randomly resampled from $\{Y^{(i)}\}_{i \in B^{d-1}_{\mathbf{u}}}$ without replacement. This implies that each summand $\mathbb{E}_{X|Y^{(\sigma(i))}}g(X, Y^{(\sigma(i))})$ for $i \in B'^{d}_{\mathbf{u}{:}p}$ is an unbiased estimator of its average over $B^{d-1}_{\mathbf{u}}$. Therefore, the inner expectation above corresponds to the variance of an unbiased estimator that uses $2^{m-d}$ samples (without replacement) to estimate the expectation of a finite population of size $2^{m-d+1}$. It follows from this argument that
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ & \leq
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}\sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}\frac{2^{m-d+1}-2^{m-d}}{2^{m-d+1}-1}\cdot
        \frac{1}{2^{m-d}}
    \\ &\quad\quad \times
        \frac{1}{2^{m-d+1}}
            \sum_{i \in B^{d-1}_{\mathbf{u}}}
            \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{j \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(j)}}
                g\left(
                    X, Y^{(j)}
                \right)
            -
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2
    \\ &=
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^m-2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
            \frac{1}{2^{m-d+1}}
            \sum_{i \in B^{d-1}_{\mathbf{u}}}
            \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{j \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(j)}}
                g\left(
                    X, Y^{(j)}
                \right)
            -
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2
    \\ &\leq
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{m-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \mathbb{E}_{X|Y^{(j)}}
            g\left(
                X, Y^{(j)}
            \right)
        \right\|_2^2
    \\ &\leq
        \alpha_1^2\beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{m-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \\ &\leq
        \alpha_1^2\beta^2
        \frac{2^{d-1}}{2^{m-1}}\cdot
        \frac{2K}{2^{(d-1)/K}}
        \leq
        \alpha_1^2
        \beta^2
        \frac{2K}{2^{(m-1)/K}},
    \end{align}
    in which we have used the condition on $g$ (see also Remark~\ref{rem:T_k}) and Lemma~\ref{lem}. In this way, the first term of \eqref{eq:main_theorem_three_terms} is bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (m+1)
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    +
        (m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ &\leq
        \frac{m+1}{2^m}
        \mathbb{V}_{Y}
        f\left(
            \mathbb{E}_{X|Y}
            g(X, Y)
        \right)
    +
        (m+1) \sum_{d=1}^{m}\alpha_1^2
        \beta^2
        \frac{2K}{2^{(m-1)/K}}
    =
        O\left(
            \frac{m^2}{2^{m/K}}
        \right).
    \end{align}

\noindent \underline{A bound on the second term of \eqref{eq:main_theorem_three_terms}:}
    Next we show a bound on the second term of \eqref{eq:main_theorem_three_terms}. Using Cauchy–Schwarz inequality, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        +
            \sum_{d=1}^{m}
               \left( \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
                \right)
        -
            \sum_{d=1}^{m}
               \left( \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
                \right)
        \right)^2
    \\ &\leq
       (m+1) \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &\quad 
        +
       (m+1) \sum_{d=1}^{m}\mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2.
    \end{align}
    The first term on the right-most side above can be bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \alpha_1^2
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left\|
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right\|_2^2
    \\ &=
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{X|Y^{(i)}}
        g\left(
            X, Y^{(i)}
        \right)
        =
        \frac{\alpha_1^2}{2^m}
        \mathbb{E}_{Y}        \mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right),
    \end{align}
    where the first inequality follows from Jensen's inequality and the second inequality follows from the first condition of $f$. Regarding each summand of the second term, let us introduce a bijection $s^*: \{1,\dots,2^m\} \to \{1,\dots,2^m\}$, which is also locally bijective between $B^{d}_{\mathbf{u}}$ and $B'^{d}_{\mathbf{u}}$, i.e., $s^*(B^{d}_{\mathbf{u}})=B'^{d}_{\mathbf{u}}$ holds for all $\mathbf{u}\in \{0,1\}^d$. Then, by using the first and second conditions on $f$ and Cauchy–Schwarz inequality, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \frac{1}{2^d}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    \mathbb{E}_{X|Y^{(i)}}
                    g\left(
                        X, Y^{(i)}
                    \right)
                \right)
            -
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            \right.
        \right.
    \\ &\quad\quad
        \left.
        -
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    \mathbb{E}_{X|Y^{(s^*(i))}}
                    g\left(
                        X, Y^{(s^*(i))}
                    \right)
                \right)
            +
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(s^*(i))}, Y^{(s^*(i))}
                    \right)
                \right)
        \right)^2
    \\ &\leq
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left(
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right.
    \\ &\quad\quad
        \left.
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(s^*(i))}}
                g\left(
                    X, Y^{(s^*(i))}
                \right)
            \right)
        +
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(s^*(i))}, Y^{(s^*(i))}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left(
            \alpha_1
            \left\|
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            -
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right.
        \right.
    \\ &\quad\quad
        \left.
            \left.
            -
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(s^*(i))}}
                g\left(
                    X, Y^{(s^*(i))}
                \right)
            +
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(s^*(i))}, Y^{(s^*(i))}
                \right)
            \right\|_2
        \right.
    \\ &\quad\quad
        \left.
        +
            \alpha_2
            \left\|
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            -
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right\|_2
        \right.
    \\ &\quad\quad\quad
        \left. \times
            \left\|
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            -
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(s^*(i))}}
                g\left(
                    X, Y^{(s^*(i))}
                \right)
            \right\|_2
        \right)^2
    \\ &\leq
        2
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left\|
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right.
    \\ &\quad\quad
        \left.
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(s^*(i))}}
            g\left(
                X, Y^{(s^*(i))}
            \right)
        +
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(s^*(i))}, Y^{(s^*(i))}
            \right)
        \right\|_2^2
    \\ &\quad\quad
    +
        2
        \alpha_2^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left\|
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right\|_2^2
    \\ &\quad\quad\quad 
        \times
        \left\|
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(s^*(i))}}
            g\left(
                X, Y^{(s^*(i))}
            \right)
        \right\|_2^2
    \\ &\leq
        2
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left\|
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right.
    \\ &\quad\quad
        \left.
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(s^*(i))}}
            g\left(
                X, Y^{(s^*(i))}
            \right)
        +
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(s^*(i))}, Y^{(s^*(i))}
            \right)
        \right\|_2^2
    \\ &\quad\quad
    +
        2
        \alpha_2^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \left\|
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            -
                \mathbb{E}_{X|Y^{(s^*(i))}}
                g\left(
                    X, Y^{(s^*(i))}
                \right)
            \right\|_2^2
        \right)
    \\ &\quad\quad\quad \times
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left\|
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right\|_2^2
    \\ &\leq
        2
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \tg{\frac{2}{2^{2(m-d)}} \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \left\|
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        -
            g\left(
                X^{(s^*(i))}, Y^{(s^*(i))}
            \right)
        \right\|_2^2}
    \\ &\quad\quad
    +
        2
        \alpha_2^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            \left\|
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            -
                \mathbb{E}_{X|Y^{(s^*(i))}}
                g\left(
                    X, Y^{(s^*(i))}
                \right)
            \right\|_2^2
        \right)
    \\ &\quad\quad\quad \times
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{V}_{X|Y^{(i)}}
        g\left(
            X, Y^{(i)}
        \right)
    \\ &\leq
        2
        \alpha_1^2
        \beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|^2_2
    \\ &\quad\quad
    +
        2
        \alpha_2^2
        \beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|_2^2
        \right)
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{V}_{X|Y^{(i)}}
        g\left(
            X, Y^{(i)}
        \right)
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|_2^2
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}\cdot
        \frac{2K}{2^{(d-1)/K}}
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{2K}{2^{(m-1)/K}}.
    \end{align}

    Therefore, the second term of \eqref{eq:main_theorem_three_terms} is bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
       (m+1) \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &\quad\quad
        +
       (m+1) \sum_{d=1}^{m}\mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ & \leq
        (m+1)\frac{\alpha_1^2}{2^m}
        \mathbb{E}_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)+(m+1)\sum_{d=0}^{m-1}2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{2K}{2^{(m-1)/K}}
    \\  &=
        O\left(
            \frac{m^2}{2^{m/K}}
        \right).
    \end{align}

\noindent \underline{A bound on the third term of \eqref{eq:main_theorem_three_terms}:}
    Finally a bound on the third term of \eqref{eq:main_theorem_three_terms} is bounded from above as follows.
    \begin{align}
    &\quad
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (2m+1)\sum_{d=0}^{m}\mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}\left( \hat{P}_{\mathrm{out}}^{(d,m-d)}-\hat{P}^{(d,m-d)}\right)^2
    \\ &\quad\quad 
        + (2m+1)\sum_{d=1}^{m}\mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}\left( \hat{Q}_{\mathrm{out}}^{(d,m-d)}-\hat{Q}^{(d,m-d)}\right)^2
    \\ &=
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
    \\ &\quad\quad
        \left(
            \frac{1}{2^d}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            -
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            \right)
        \right)^2
    \\ &\quad\quad
    +
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
    \\ &\quad\quad\quad
        \left(
            \frac{1}{2^d}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B'^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            -
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B'^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            \right)
        \right)^2
    \\ &=
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        f\left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right)
    \\ &\quad
    +
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        f\left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B'^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right)
    \\ &\leq
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        \frac{1}{2^{m-d}}
        \sum_{i \in B'^d_{\mathbf{u}}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B'^d_{\mathbf{u}}}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \frac{1}{2^m}
        \alpha_1^2
        (2m+1)^2\,
        \mathbb{E}_{Y}
        \mathbb{V}_{X|Y}
        g(X, Y).
    \end{align}
    Combining the respective upper bound on each of the three terms of \eqref{eq:main_theorem_three_terms}, we complete the proof of the theorem. 
\end{proof}

Our theoretical result shows that the MSE of our proposed method decays at least as fast as $N^{-1/K}(\log N)^2$. In comparison, the authors' previous method in \cite{hironaka2023efficient} has an upper bound of $O(N^{-1/2K})$ under the same conditions as in Theorem~\ref{thm:main}. Thus, our proposed method has a faster rate of convergence in terms of upper bounds. The rate $N^{-1/K}(\log N)^2$ indicates that our method is efficient when the dimensionality of the outer random variable $K$ is small. However, due to the exponential dependence on $K$, our method may not be efficiently applicable to high-dimensional problems, and estimating nested expectations may suffer from the curse of dimensionality.

In fact, a similar exponential dependence of the approximation error on $K$ also appears in other studies, such as \cite{hong2017kernel} and \cite{broto2020variance}, in which nested expectations are estimated without sampling from the inner conditional distribution. This implies that the curse of dimensionality is a common issue in estimating nested expectations without inner conditional sampling. Further studies could investigate whether it is possible to overcome the curse of dimensionality or not.


==> 30-theoretical_ver2.tex <==

\section{Theoretical Analysis}\label{sec:theoretical}

In this section, we provide an upper bound on the MSE of our proposed method (Algorithm~\ref{alg:proposed}). We begin by introducing our notation for variance. Throughout this section, given a random vector $Z$, we define the variance of $Z$ as the trace of the covariance matrix of $Z$ and denote it by $\mathbb{V}_{\rho(Z)}Z$. This notation also applies to the case of conditional variance, where we use an appropriate subscript to represent the underlying conditional distribution. Moreover, whenever the underlying probability distribution is clear from the context, we omit the subscript from $\mathbb{E}$ or $\mathbb{V}$ or simply denote the underlying random variables for the subscript instead of the probability distribution. 

As the main theoretical result of this paper, we show the following theorem.
\begin{theorem}\label{thm:main}
    Let $m\in \mathbb{N}$ and $N = 2^m$.
    Assume that $\sup_{Y}\mathbb{V}_{X|Y}g\left(X, Y\right)<\infty$, and there exist positive constants $\alpha_1, \alpha_2, \beta$ and functions $\mathcal{T}_k: \mathbb{R}\to [0,1]$ for all $k=1,\dots, K$, such that
    \begin{enumerate}
        \item \tg{$\left| f\left( g \right) - f\left( g' \right) \right| \leq \alpha_1 \left\| g-g' \right\|_2$},
        \item \tg{$\left| \mathbb{E}_hf\left( h \right) - f\left( \mathbb{E}_h h \right) \right| \leq \alpha_2 \sqrt{\mathbb{V}_h h}$,}
        \item $\left\|\mathbb{E}_{X|Y}g\left( X, Y \right) - \mathbb{E}_{X'|Y'}g\left( X', Y' \right)\right\|_2 \leq \beta\left\| \mathcal{T}(Y) - \mathcal{T}(Y') \right\|_2$,
    \end{enumerate}
    for any vectors $g, g'\in \mathbb{R}^G$, random vector $h\in \mathbb{R}^G$ and $Y, Y' \in \mathbb{R}^K$, in which we write $\mathcal{T}(Y)=(\mathcal{T}_1(Y_1),\dots,\mathcal{T}_K(Y_K)).$
    Then we have
    \begin{align}
        \mathbb{E}(I - \hat{I})^2
    =
        O\left( \frac{(\log N)^2}{N^{1/K}} \right).
    \end{align}
\end{theorem}

Before going into the proof of the theorem, let us make some remarks.
\begin{remark}\label{rem:T_k}
The assumption of the existence of functions $\mathcal{T}_k$ may appear artificial. To argue that this is not the case, let us consider the following change of variables: for $k=1,\dots,K$, let $F_k$ denote the cumulative marginal distribution function of the outer variable $Y_k$ and let $Z_k=F_k(Y_k)$. This transformation ensures that $0 \leq Z_k \leq 1$. Therefore, a natural choice for $\mathcal{T}_k$ is $\mathcal{T}_k=F_k$.
\end{remark}

\begin{remark}\label{rem:holder}
When the outer function $f$ satisfies the first condition, it implies that
\begin{align*}
aaa    
\end{align*}
holds for any vectors $g, h\in \mathbb{R}^G$.

Let us consider the problem setting for estimating EVSI, that is, the case where $f=\max_{d\in D}$ for a set $D$ with finite cardinality $G$. It can be checked that the above condition on $f$ is satisfied:
\begin{align*}
    \left| \max_{1\leq j\leq G}g_j-\max_{1\leq j\leq G}h_j\right|\leq \max_{1\leq j\leq G}\left| g_j-h_j\right|\leq \sum_{j=1}^{G}\left| g_j-h_j\right|\leq \sqrt{G}\, \|g-h\|_2,
\end{align*}
where the last inequality follows from Cauchy–Schwarz inequality. However, the first condition on $f$ in Theorem~\ref{thm:main} seems to be not satisfied in general, so that our result does not necessarily cover the problem setting for estimating EVSI. Therefore, discussing whether the conditions given in Theorem~\ref{thm:main} can be weakened such that the theorem covers the EVSI setting remains an open problem.
\end{remark}

As a preparation for proving Theorem~\ref{thm:main}, we present the following lemma.
\begin{lemma}\label{lem}
    Let $m \in \mathbb{N}$, and let $\{(X^{(i)}, Y^{(i)})\}_{1 \leq i \leq 2^m}$ be a set of i.i.d.\ random samples from the joint distribution $\rho(X,Y)$. For $d \in \{0, \dots, m\}$ and $\mathbf{u} \in \{0,1\}^d$, let $B^{d}_{\mathbf{u}}$ be constructed as described in Algorithm~\ref{alg:proposed}. Then, assuming the existence of functions $\mathcal{T}_k: \mathbb{R}\to [0,1]$ for all $k=1,\dots, K$  we have for any $d \in \{0, \dots, m\}$
    \begin{align}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \leq
        \frac{2K}{2^{d/K}}.
    \end{align}
\end{lemma}

\begin{proof}
    Let $N=2^m$. For $d \in \{0, \dots, m\}$ and $k\in \{1,\dots, K\}$, define
    \begin{align}
        W_{d, k}
    =
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right).
    \end{align}
    
    If $d = 0$, it is easy to see from the definition $B^0_{\emptyset}:=\{1,\dots,2^m\}$ that
    \begin{align}
        W_{0, k}
    =
        \max_{i \in B^0_{\emptyset}}
        \mathcal{T}_k(Y_k^{(i)})
    -
        \min_{i \in B^0_{\emptyset}}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \max_{ i=1, \dots, 2^m }
        \mathcal{T}_k(Y_k^{(i)})
    -
        \min_{ i=1, \dots, 2^m }
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        1
    \end{align}
    holds for all $k\in\{1,\dots,K\}$.
    
    Otherwise if $1 \leq d \leq m$, it follows from the construction of $B^{d}_{\mathbf{u}}$'s that, for $k = (d-1 \bmod K) +1 \in \{1,\dots,K\}$, we have
    \begin{align}
    & 
        \min_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \min_{i \in B_{\mathbf{u}{:}0}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}0}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \\ &\quad \quad \leq
        \min_{i \in B_{\mathbf{u}{:}1}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}1}^d}
        \mathcal{T}_k(Y_k^{(i)})
    =
        \max_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \end{align}
    for all $\mathbf{u} \in \{0, 1\}^{d-1}$. Therefore, we obtain
    \begin{align}
        W_{d, k} &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        +
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        \right)
    \\ &\leq
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \max_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right) =
        \frac{1}{2}
        W_{d-1, k}.
    \end{align}
    For $k \neq (d-1 \bmod K) +1 $, we have
    \begin{align}
    \quad
        \min_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \min_{i \in B_{\mathbf{u}{:}p}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}{:}p}^d}
        \mathcal{T}_k(Y_k^{(i)})
    \leq
        \max_{i \in B_{\mathbf{u}}^{d-1}}
        \mathcal{T}_k(Y_k^{(i)})
    \end{align}
    for all $\mathbf{u} \in \{0, 1\}^{d-1}$ and $p \in \{0, 1\}$. Therefore, we obtain
    \begin{align}
     W_{d, k} &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}0}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        +
            \left(
                \max_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            -
                \min_{i \in B^d_{\mathbf{u}{:}1}}
                \mathcal{T}_k(Y_k^{(i)})
            \right)
        \right)
    \\ &\leq
        \frac{2}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \left(
            \max_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^{d-1}_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right) =
        W_{d-1, k}.
    \end{align}
    Using these results, it can be concluded that, for any $k\in \{1,\dots,K\}$, we have
    \begin{align}
        W_{d, k} \leq \begin{cases} 1 & \text{if $d < K$,}\\ W_{d-K, k}/2 & \text{otherwise.} \end{cases}
    \end{align}
    so that it holds that
    \begin{align}
            W_{d, k}
        \leq
            \frac{1}{2^{\lfloor d/K \rfloor}}
            W_{d-K\lfloor d/K \rfloor, k}
        \leq
            \frac{1}{2^{\lfloor d/K \rfloor}}
        \leq
            \frac{2}{2^{d/K}},
    \end{align}
    for any $1\leq d\leq m$. Note that this upper bound on $W_{d, k}$ also applies to the case $d=0$.

    Recalling the assumption that $0 \leq \mathcal{T}_k(Y_k) \leq 1$ for any $Y_k$ for all $k=1,\dots, K$, we have for any $d \in \{0, \dots, m\}$
    \begin{align}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2 &\leq
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_1
    \\ &\leq
        \frac{1}{2^d}
        \sum_{k=1}^{K}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \max_{i, j \in B^d_{\mathbf{u}}}
        \left|
            \mathcal{T}_k(Y_k^{(i)})
        -
            \mathcal{T}_k(Y_k^{(j)})
        \right|
    \\ &=
        \frac{1}{2^d}
        \sum_{k=1}^{K}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            \max_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        -
            \min_{i \in B^d_{\mathbf{u}}}
            \mathcal{T}_k(Y_k^{(i)})
        \right)
    \\ &=
        \sum_{k=1}^{K}
        W_{d, K} \leq
        \frac{2K}{2^{d/K}},
    \end{align}
    which completes the proof of the lemma.
\end{proof}

Let us now prove Theorem~\ref{thm:main}.

%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
\begin{proof}[Proof of Theorem~\ref{thm:main}]
    Together with the notation used in Section~\ref{sec:method}, we further introduce the following notation in this proof:
    \begin{align*}
        \hat{P}_{\mathrm{in}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}f\left(\frac{1}{2^{m-d}}\sum_{i \in B^d_{\mathbf{u}}}\mathbb{E}_{X|Y^{(i)}}g\left(X, Y^{(i)}\right)\right), \\
        \hat{Q}_{\mathrm{in}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}f\left(\frac{1}{2^{m-d}}\sum_{i \in B'^d_{\mathbf{u}}}\mathbb{E}_{X|Y^{(i)}}g\left(X, Y^{(i)}\right)\right), \\
        \hat{P}_{\mathrm{out}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}\mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}f\left(\frac{1}{2^{m-d}}\sum_{i \in B^d_{\mathbf{u}}}g\left(X^{(i)}, Y^{(i)}\right)\right), \\
        \hat{Q}_{\mathrm{out}}^{(d,m-d)} & = \frac{1}{2^d}\sum_{\mathbf{u} \in \{0, 1\}^d}\mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}f\left(\frac{1}{2^{m-d}}\sum_{i \in B'^d_{\mathbf{u}}}g\left(X^{(i)}, Y^{(i)}\right)\right).
    \end{align*}
    Then, by using a trivial inequality $(a+b+c)^2\leq 3(a^2+b^2+c^2)$ for any $a,b,c\in \mathbb{R}$, which follows immediately from Cauchy–Schwarz inequality, we have
    \begin{align}
    &\quad
        \mathbb{E}(I - \hat{I})^2
    \\ &=
        \mathbb{E}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        3
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\quad\quad
    +
        3
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\quad\quad
    +
        3
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2.\label{eq:main_theorem_three_terms}
    \end{align}
In the following, we derive an upper bound on each of the three terms of \eqref{eq:main_theorem_three_terms}. 

\noindent \underline{A bound on the first term of \eqref{eq:main_theorem_three_terms}:}
We start by considering the first term. Applying Cauchy–Schwarz inequality again, we obtain
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &=\mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        -
            \sum_{d=1}^{m}
                \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (m+1)
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    +
        (m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2.
    \end{align}
For the first term on the right-most side above, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
             \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            f\left(
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        \right)^2 
        =
        \frac{1}{2^m}
        \mathbb{V}_{Y}
        f\left(
            \mathbb{E}_{X|Y}
            g(X, Y)
        \right).
    \end{align}
Regarding each summand of the second term, applying Jensen's inequality and using the condition on $f$ (see also Remark~\ref{rem:holder}) and the exchangeability of the samples $\{Y^{(i)}\}_i$, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
        \frac{1}{2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
            \left(
            f\left(
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
            \right.
        \right.
    \\ & \quad\quad
        -
            \left.
            \left.
            \frac{1}{2}
            \sum_{p \in \{0, 1\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
            \right)
        \right)^2
    \\ & \leq 
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}
    \\ & \quad\quad
        \left(
            f\left(
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ & \leq 
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}
        \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        -
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        \right\|_2^2
    \\ & =
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}\sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}\mathbb{E}_{\sigma|\{Y^{(i)}\}}
    \\ &\quad\quad
        \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{i \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        -
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^{d}_{\mathbf{u}{:}p}}
                \mathbb{E}_{X|Y^{(\sigma(i))}}
                g\left(
                    X, Y^{(\sigma(i))}
                \right)
        \right\|_2^2,
    \end{align}
    where, conditioned on $\{Y^{(i)}\}$, $\sigma$ denotes a random permutation of the indices $1,\dots,2^m$ such that $\sigma(B^{d-1}_{\mathbf{u}})=B^{d-1}_{\mathbf{u}}$. By construction of $B'^{d}_{\mathbf{u}{:}p}$ and because of the restriction $\sigma(B^{d-1}_{\mathbf{u}})=B^{d-1}_{\mathbf{u}}$, the set  $\{Y^{(\sigma(i))}\}_{i \in B'^{d}_{\mathbf{u}{:}p}}$ can be regarded as a set of the samples randomly resampled from $\{Y^{(i)}\}_{i \in B^{d-1}_{\mathbf{u}}}$ without replacement. This implies that each summand $\mathbb{E}_{X|Y^{(\sigma(i))}}g(X, Y^{(\sigma(i))})$ for $i \in B'^{d}_{\mathbf{u}{:}p}$ is an unbiased estimator of its average over $B^{d-1}_{\mathbf{u}}$. Therefore, the inner expectation above corresponds to the variance of an unbiased estimator that uses $2^{m-d}$ samples (without replacement) to estimate the expectation of a finite population of size $2^{m-d+1}$. It follows from this argument that
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ & \leq
        \alpha_1^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d}}\sum_{\mathbf{u} \in \{0, 1\}^{d-1}}\sum_{p \in \{0, 1\}}\frac{2^{m-d+1}-2^{m-d}}{2^{m-d+1}-1}\cdot
        \frac{1}{2^{m-d}}
    \\ &\quad\quad \times
        \frac{1}{2^{m-d+1}}
            \sum_{i \in B^{d-1}_{\mathbf{u}}}
            \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{j \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(j)}}
                g\left(
                    X, Y^{(j)}
                \right)
            -
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2
    \\ &=
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^m-2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
            \frac{1}{2^{m-d+1}}
            \sum_{i \in B^{d-1}_{\mathbf{u}}}
            \left\|
                \frac{1}{2^{m-d+1}}
                \sum_{j \in B^{d-1}_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(j)}}
                g\left(
                    X, Y^{(j)}
                \right)
            -
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2
    \\ &\leq
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{m-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \mathbb{E}_{X|Y^{(j)}}
            g\left(
                X, Y^{(j)}
            \right)
        \right\|_2^2
    \\ &\leq
        \alpha_1^2\beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{m-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \\ &\leq
        \alpha_1^2\beta^2
        \frac{2^{d-1}}{2^{m-1}}\cdot
        \frac{2K}{2^{(d-1)/K}}
        \leq
        \alpha_1^2
        \beta^2
        \frac{2K}{2^{(m-1)/K}},
    \end{align}
    in which we have used the condition on $g$ and Lemma~\ref{lem}. In this way, the first term of \eqref{eq:main_theorem_three_terms} is bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}g(X, Y)
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (m+1)
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \mathbb{E}_Y
            f\left(
                \mathbb{E}_{X|Y}
                g(X, Y)
            \right)
        -
            \hat{P}_{\mathrm{in}}^{(m,0)}
        \right)^2
    +
        (m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d-1,m-d+1)}
            -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
        \right)^2
    \\ &\leq
        \frac{m+1}{2^m}
        \mathbb{V}_{Y}
        f\left(
            \mathbb{E}_{X|Y}
            g(X, Y)
        \right)
    +
        (m+1) \sum_{d=1}^{m}\alpha_1^2
        \beta^2
        \frac{2K}{2^{(m-1)/K}}
    =
        O\left(
            \frac{m^2}{2^{m/K}}
        \right).
    \end{align}

\noindent \underline{A bound on the second term of \eqref{eq:main_theorem_three_terms}:}
    Next we show a bound on the second term of \eqref{eq:main_theorem_three_terms}. Using Cauchy–Schwarz inequality, we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        +
            \sum_{d=1}^{m}
               \left( \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
                \right)
        -
            \sum_{d=1}^{m}
               \left( \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
                \right)
        \right)^2
    \\ &\leq
       (m+1) \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &\quad 
        +
       (m+1) \sum_{d=1}^{m}\mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2.
    \end{align}
    The first term on the right-most side above can be bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &=
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
            f\left(
                \frac{1}{2^m}
                \sum_{i=1}^{2^m}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \alpha_1^2
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left\|
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            \mathbb{E}_{X|Y^{(i)}}
            g\left(
                X, Y^{(i)}
            \right)
        -
            \frac{1}{2^m}
            \sum_{i=1}^{2^m}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right\|_2^2
    \\ &=
        \alpha_1^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{X|Y^{(i)}}
        g\left(
            X, Y^{(i)}
        \right)
        =
        \frac{\alpha_1^2}{2^m}
        \mathbb{E}_{Y}        \mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right),
    \end{align}
    where the first inequality follows from Jensen's inequality and the second inequality follows from the condition of $f$ (cf.\ Remark~\ref{rem:holder}). Regarding each summand of the second term, %by using the condition on $f$ and Cauchy–Schwarz inequality, 
    we have
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ & =
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \frac{1}{2^{d}}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right.
        \right.
    \\ &\quad\quad
        \left.
        \left.
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        +
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)
        \right)^2.
    \end{align}
    By applying the mean value theorem for functions with multiple variables, regarding the second and fourth summands above, there exist vectors $s_{\mathbf{u}},t_{\mathbf{u}}\in [0,1]^G$ such that
    \begin{align*}
        & f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right) 
        \\& = 
        f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right) 
        \\ &\quad\quad +
                \nabla f
                \left( s_{\mathbf{u}}\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
                +
                (\boldsymbol{1}-s_{\mathbf{u}})\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
                \right)
        \\ &\quad\quad\quad\quad \cdot
            \left(
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right),
    \end{align*}
    and
    \begin{align*}
        & f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right) 
        \\& = 
        f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right) 
        \\ &\quad\quad +
                \nabla f
                \left( t_{\mathbf{u}}\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
                +
                (\boldsymbol{1}-t_{\mathbf{u}})\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
                \right)
        \\ &\quad\quad\quad\quad \cdot
            \left(
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right),
    \end{align*}
    respectively. Using these equalities, we obtain
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ & =
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \frac{1}{2^{d}}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            \right.
    \\ &\quad\quad \left[
                \nabla f
                \left( s_{\mathbf{u}}\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
                +
                (\boldsymbol{1}-s_{\mathbf{u}})\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
                \right)
                \right.
        \\ &\quad\quad\quad\quad \cdot
            \left(
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        \\ &\quad\quad
                -\nabla f
                \left( t_{\mathbf{u}}\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
                +
                (\boldsymbol{1}-t_{\mathbf{u}})\cdot \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
                \right)
        \\ &\quad\quad\quad\quad \cdot
            \left.
            \left.
            \left(
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
            \right]
            \right)^2
        \\ & \leq
        \mathbb{E}_{\{Y^{(i)}\}}
            \frac{\alpha_2^2}{2^{d-1}}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
                   \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
        \\ &\quad\quad \left(
            \left\|
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2+
        \right.
        \\ &\quad\quad
        +
            \left.
            \left\|
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            -
            \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right\|_2^2
            \right)
        \\ & =
        \mathbb{E}_{\{Y^{(i)}\}}
            \frac{\alpha_2^2}{2^{d-1}}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
                  \left( \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}\left( \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)\right)
                +
                \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}\left( \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)\right)
                \right)
    \end{align}

    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ &\leq
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        -
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right.
    \\ &\quad\quad
        \left.
        -
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
            \right)
        +
        \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
            f\left(
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                g\left(
                    X^{(i)}, Y^{(i)}
                \right)
            \right)
        \right)^2
    \\ &\leq
        \alpha^2\mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d-2}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left\|
                \frac{1}{2^{m-d}}
                \sum_{i \in B^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        -
                \frac{1}{2^{m-d}}
                \sum_{i \in B'^d_{\mathbf{u}}}
                \mathbb{E}_{X|Y^{(i)}}
                g\left(
                    X, Y^{(i)}
                \right)
        \right\|_2^2
    \\ &\leq
        2
        \alpha_1^2
        \beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|^2_2
    \\ &\quad\quad
    +
        2
        \alpha_2^2
        \beta^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \left(
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|_2^2
        \right)
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{V}_{X|Y^{(i)}}
        g\left(
            X, Y^{(i)}
        \right)
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^d}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(s^*(i))})
        \right\|_2^2
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{d-1}}
        \sum_{\mathbf{u} \in \{0, 1\}^{d-1}}
        \max_{i, j \in B^{d-1}_{\mathbf{u}}}
        \left\|
            \mathcal{T}(Y^{(i)})
        -
            \mathcal{T}(Y^{(j)})
        \right\|_2^2
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{1}{2^{m-d}}\cdot
        \frac{2K}{2^{(d-1)/K}}
    \\ &\leq
        2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{2K}{2^{(m-1)/K}}.
    \end{align}

    Therefore, the second term of \eqref{eq:main_theorem_three_terms} is bounded above by
    \begin{align}
    &\quad
        \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
       (m+1) \mathbb{E}_{\{Y^{(i)}\}}
        \left(
            \hat{P}_{\mathrm{in}}^{(0,m)}-\hat{P}_{\mathrm{out}}^{(0,m)}
        \right)^2
    \\ &\quad\quad
        +
       (m+1) \sum_{d=1}^{m}\mathbb{E}_{\{Y^{(i)}\}}
        \left(
                \hat{P}_{\mathrm{in}}^{(d,m-d)}
            -
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
        -
                \hat{Q}_{\mathrm{in}}^{(d,m-d)}
            +
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
        \right)^2
    \\ & \leq
        (m+1)\frac{\alpha_1^2}{2^m}
        \mathbb{E}_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)+(m+1)\sum_{d=0}^{m-1}2\beta^2
        \left(
            \alpha_1^2
        +
            \alpha_2^2
            \sup_{Y}\mathbb{V}_{X|Y}
        g\left(
            X, Y
        \right)
        \right)
        \frac{2K}{2^{(m-1)/K}}
    \\  &=
        O\left(
            \frac{m^2}{2^{m/K}}
        \right).
    \end{align}

\noindent \underline{A bound on the third term of \eqref{eq:main_theorem_three_terms}:}
    Finally a bound on the third term of \eqref{eq:main_theorem_three_terms} is bounded from above as follows.
    \begin{align}
    &\quad
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
        \left(
            \left(
                \sum_{d=0}^{m}
                \hat{P}_{\mathrm{out}}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}_{\mathrm{out}}^{(d,m-d)}
            \right)
        -
            \left(
                \sum_{d=0}^{m}
                \hat{P}^{(d,m-d)}
            -
                \sum_{d=1}^{m}
                \hat{Q}^{(d,m-d)}
            \right)
        \right)^2
    \\ &\leq
        (2m+1)\sum_{d=0}^{m}\mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}\left( \hat{P}_{\mathrm{out}}^{(d,m-d)}-\hat{P}^{(d,m-d)}\right)^2
    \\ &\quad\quad 
        + (2m+1)\sum_{d=1}^{m}\mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}\left( \hat{Q}_{\mathrm{out}}^{(d,m-d)}-\hat{Q}^{(d,m-d)}\right)^2
    \\ &=
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
    \\ &\quad\quad
        \left(
            \frac{1}{2^d}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            -
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            \right)
        \right)^2
    \\ &\quad\quad
    +
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{(X^{(i)},Y^{(i)})\}}
    \\ &\quad\quad\quad
        \left(
            \frac{1}{2^d}
            \sum_{\mathbf{u} \in \{0, 1\}^d}
            \left(
                \mathbb{E}_{\{X^{(i)}|Y^{(i)}\}}
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B'^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            -
                f\left(
                    \frac{1}{2^{m-d}}
                    \sum_{i \in B'^d_{\mathbf{u}}}
                    g\left(
                        X^{(i)}, Y^{(i)}
                    \right)
                \right)
            \right)
        \right)^2
    \\ &=
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        f\left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right)
    \\ &\quad
    +
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        f\left(
            \frac{1}{2^{m-d}}
            \sum_{i \in B'^d_{\mathbf{u}}}
            g\left(
                X^{(i)}, Y^{(i)}
            \right)
        \right)
    \\ &\leq
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        \frac{1}{2^{m-d}}
        \sum_{i \in B^d_{\mathbf{u}}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        \frac{1}{2^{m-d}}
        \sum_{i \in B'^d_{\mathbf{u}}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B^d_{\mathbf{u}}}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2d}}
        \sum_{\mathbf{u} \in \{0, 1\}^d}
        \frac{1}{2^{2(m-d)}}
        \sum_{i \in B'^d_{\mathbf{u}}}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)
        \sum_{d=0}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &\quad
    +
        \alpha_1^2
        (2m+1)
        \sum_{d=1}^{m}
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \alpha_1^2
        (2m+1)^2
        \mathbb{E}_{\{Y^{(i)}\}}
        \frac{1}{2^{2m}}
        \sum_{i=1}^{2^m}
        \mathbb{V}_{\{X^{(i)}|Y^{(i)}\}}
        g\left(
            X^{(i)}, Y^{(i)}
        \right)
    \\ &=
        \frac{1}{2^m}
        \alpha_1^2
        (2m+1)^2\,
        \mathbb{E}_{Y}
        \mathbb{V}_{X|Y}
        g(X, Y).
    \end{align}
    Combining the respective upper bound on each of the three terms of \eqref{eq:main_theorem_three_terms}, we complete the proof of the theorem. 
\end{proof}

Our theoretical result shows that the MSE of our proposed method decays at least as fast as $N^{-1/K}(\log N)^2$. In comparison, the authors' previous method in \cite{hironaka2023efficient} has an upper bound of $O(N^{-1/2K})$ under the same conditions as in Theorem~\ref{thm:main}. Thus, our proposed method has a faster rate of convergence in terms of upper bounds. The rate $N^{-1/K}(\log N)^2$ indicates that our method is efficient when the dimensionality of the outer random variable $K$ is small. However, due to the exponential dependence on $K$, our method may not be efficiently applicable to high-dimensional problems, and estimating nested expectations may suffer from the curse of dimensionality.

In fact, a similar exponential dependence of the approximation error on $K$ also appears in other studies, such as \cite{hong2017kernel} and \cite{broto2020variance}, in which nested expectations are estimated without sampling from the inner conditional distribution. This implies that the curse of dimensionality is a common issue in estimating nested expectations without inner conditional sampling. Further studies could investigate whether it is possible to overcome the curse of dimensionality or not.

